LaDDer: Latent Data Distribution Modelling with a Generative Prior

In this paper, we show that the performance of a learnt generative model is closely related to the model's ability to accurately represent the inferred \textbf{latent data distribution}, i.e. its topology and structural properties. We propose LaDDer to achieve accurate modelling of the latent data distribution in a variational autoencoder framework and to facilitate better representation learning. The central idea of LaDDer is a meta-embedding concept, which uses multiple VAE models to learn an embedding of the embeddings, forming a ladder of encodings. We use a non-parametric mixture as the hyper prior for the innermost VAE and learn all the parameters in a unified variational framework. From extensive experiments, we show that our LaDDer model is able to accurately estimate complex latent distribution and results in improvement in the representation quality. We also propose a novel latent space interpolation method that utilises the derived data distribution.

==> vAlgorithm.tex <==
% Two Column Compatible, Variable Width Algorithm Environments
% Written by Daniel Herber
% Based on modifications to the stack exchange answer at
% http://tex.stackexchange.com/questions/23296/setting-caption-rule-width-in-algorithm2e-algs/39574

% inputs
% 1 : float specifiers (htbp!)
% 2 : algorithm width (length)
% 3 : indent width (length)

% column environment
% \begin{vAlgorithm}[float specifiers]{algorithm width}{indent width}
% \end{vAlgorithm}

% page environment
% \begin{vAlgorithm*}[float specifiers]{algorithm width}{indent width}
% \end{vAlgorithm*}

% required packages
\usepackage{algorithm2e}
\usepackage{etoolbox}
\usepackage{xstring}
\usepackage{calc}
 
% define lengths
\newlength{\xalgowidth}
\newlength{\xalgoremainder}
\newlength{\xindentwidth}

% define vAlgorithm* environment
\newenvironment{vAlgorithm*}[3][]{% before
  \setlength{\xalgowidth}{#2} % set algorithm width from second input
  \setlength{\xindentwidth}{#3} % set indent width from third input
  \setlength{\xalgoremainder}{\textwidth-\xalgowidth} % calculate indent to center the float
  \SetCustomAlgoRuledWidth{\xalgowidth} % set the rule width
  \IncMargin{\xindentwidth}
  \begin{algorithm*}[#1]
}% end before
{% after
  \end{algorithm*} 
  \DecMargin{\xindentwidth}
}% end after

% define vAlgorithm environment
\newenvironment{vAlgorithm}[3][]{% before
  \setlength{\xalgowidth}{#2} % set algorithm width from second input
  \setlength{\xindentwidth}{#3} % set indent width from third input
  \setlength{\xalgoremainder}{\columnwidth-\xalgowidth} % calculate indent to center the float
  \SetCustomAlgoRuledWidth{\xalgowidth} % set the rule width
  \IncMargin{\xindentwidth}
  \begin{algorithm}[#1] % column
}% end before
{% after
  \end{algorithm} % column
  \DecMargin{\xindentwidth}
}% end after

% redefine algorithm commands
\makeatletter
\patchcmd{\@algocf@start}{%
\begin{lrbox}{\algocf@algobox}%
}{%
\rule{0.5\xalgoremainder}{\z@}% indent
\begin{lrbox}{\algocf@algobox}%
\begin{minipage}{\xalgowidth}%
}{}{}
\patchcmd{\@algocf@finish}{%
\end{lrbox}%
}{%
\end{minipage}%
\end{lrbox}%
}{}{}
\makeatother
